No Regret Sample Selection with Noisy Labels

Deep neural networks (DNNs) suffer from noisy-labeled data because of the risk of overfitting. To avoid the risk, in this paper, we propose a novel DNN training method with sample selection based on adaptive k-set selection, which selects k (< n) clean sample candidates from the whole n noisy training samples at each epoch. It has a strong advantage of guaranteeing the performance of the selection theoretically. Roughly speaking, a regret, which is defined by the difference between the actual selection and the best selection, of the proposed method is theoretically bounded, even though the best selection is unknown until the end of all epochs. The experimental results on multiple noisy-labeled datasets demonstrate that our sample selection strategy works effectively in the DNN training; in fact, the proposed method achieved the best or the second-best performance among state-of-the-art methods, while requiring a significantly lower computational cost. The code is available at https://github.com/songheony/TAkS.

==> texts/trush.tex <==
\subsection{Noisiness feedback function}
\label{subsec:noisiness}
The key to \Ours is the reasonable feedback function which gives $\btheta_t$.
In this study, as a feedback function, we attempt to evaluate the ``noisiness'' of individual samples based on the classification behavior of the DNN under training. If the $i$th sample 
$(x_i, y_i)$ is suspected as an incorrectly-labeled sample, its noisiness $\theta_{i,t}$ becomes large.
Specifically, we consider the following feedback function:
\begin{align}
\label{align:loss}
\theta_{i,t} = \frac{1- \mathrm{is}(f_t(x_i)= y_i)p(f_t(x_i))}{2},
\end{align}
where $f_t$ is the DNN trained by $t$ epochs and $f_t(x_i)$ is the predicted label of $x_i$.  
The function $\mathrm{is}(\cdot)$ returns $+1$ if $\cdot$ is true and returns $-1$ otherwise, and $p$ denotes the probability (i.e., softmax output) for the predicted label $f_t(x_i)$.
\par
This function is designed to evaluate the following straightforward expectation: the samples that are correctly predicted with higher
confidence should be cleaner (with a correct label), and the samples that are wrongly predicted with higher confidence should be noisier (i.e., with a wrong label). Note that \Ours can choose any noisiness feedback function other than (\ref{align:loss}); fortunately, the theoretical support (i.e., regret bound in Section~\ref{sec:theo}) holds regardless of the choice.
\par






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% old version of method.tex
\subsection{Basic settings}
We assume a DNN-based classifier that can output the class-wise probability, and the classifier is trained with noisy-labeled samples. Let $(x_1, y_1), \ldots, (x_n, y_n)$ be training samples. Some of them are samples with incorrect class labels.
The goal is to obtain a DNN-based classifier $f$ that achieves high classification accuracy on a test sample set.  Note that, in the popular setup of noisy-labeled samples, the test sample set is not noisy to facilitate the final classification evaluation easier. This paper also follows the same setup.
\par
Motivated by adaptive $k$-set selection in~\ref{subsec:kset},
we consider the basic procedure of \Ours as follows:
At each epoch $t$,
\begin{enumerate}
\item Select $\bd_{t}$ from $\mathcal{D}$ by FPL with $\btheta_{t-1}$.
\item Receive feedback which represents the noisiness of each data as $\btheta_t$.
\end{enumerate}
The sample selection algorithm by FPL in \ref{subsec:algo}. For simplicity, DNN is not shown in the above steps; in practice, one epoch training of the DNN is performed with $\bd_t$ after Step 1, and then the feedback $\btheta_t$ is given in Step 2. \par
Note that our sample selection method works generally without any assumption of the generation process of the feedback.
We would like to discuss our method with leaving the generation process of the noisiness feedback as black-box until Section~\ref{sec:experiment}.
%The total selection loss $\sum_{t=1}^T \bd_t \cdot \bell_t$ corresponds to the total number of False Positive (FP).
\par
To achieve high classification performance by a DNN, the selection algorithm is required to avoid selecting noise-samples as possible in every training epoch. As noted in~\ref{subsec:kset}, The adaptive $k$-set selection strategy meets this requirement because it selects a $k$-set near to the best $k$-set at each epoch, even though the best $k$-set is unknown until the final epoch.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$k$-set selection by FPL}
\label{subsec:algo}
We present the pseudocode of \Ours in Algorithm~\ref{alg:main} for completeness. The main task is to select a promising $k$-set at each epoch. For this task,  we employ FPL~\cite{cohen2015following} as a selection algorithm for adaptive $k$-set selection. FPL is an improved version of the {\em Follow the Leader} (FTL) algorithm~\cite{hazan2016introduction}, which selects the current optimal $k$-set at epoch $t$ (i.e., the $k$-set that gives the minimum total selection loss). 
FPL selects $k$ samples based on the perturbed selection loss, in order to avoid FTL's overfitting risk and improve the regret bound. More precisely, 
Steps 7 and 8 in Algorithm~\ref{alg:main} show the $k$-set selection algorithm based on FPL, where $\boldsymbol{r}$ is a random vector~\cite{kalai2002geometric,cohen2015following} for the perturbation.
\par
The minimization operation in~(\ref{align:FPLupdate}) can be efficiently performed with $O(n)$ computations despite $|\mathcal{D}|=\binom{n}{k}$.
The term to be minimized is rewritten as follows:
$\left(\sum^{t}_{\tau=1} \bd \cdot \btheta_\tau + \eta\bd \cdot \boldsymbol{r}  \right)=\left(\sum^{t}_{\tau=1} \btheta_\tau + \eta\boldsymbol{r}\right)\cdot\bd$.
%The efficiency is derived from the fact that
Therefore, finding the optimal $\bd$ in~(\ref{align:FPLupdate}) is equivalent to finding the elements with the $k$ least perturbed total selection risk in $\left(\sum^{t}_{\tau=1} \btheta_\tau + \eta\boldsymbol{r}\right)$ and requires $O(n)$ computations for finding the top-$k$ elements from $n$ elements~\cite{musser1997introspective}. Consequently, \Ours works efficiently with just $O(n)$ computations and thus can deal with very large training sample sets.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Efficiency and versatility}
The major computational cost of \Ours comes from $O(n)$ computations for the sample selection steps (Steps 6-8 in Algorithm~\ref{alg:main}) 
and the DNN training cost with $k$ samples (Step 5). In practice, the former is much less than the latter. Consequently, \Ours requires the DNN training cost with $k~(<n)$ samples instead of $n$ samples and thus even more efficient than the standard DNN training with all $n$ samples. 
\par
Algorithm~\ref{alg:main} also shows the versatility of \Ours; we can employ an arbitrary DNN. %In fact, at Step 5, the DNN is treated as a black-box that gives only feedback to estimate the noisiness $\theta_{i,t}$ for each sample at each epoch. 
In the later experiment, we use several different neural networks in \Ours. 

\begin{algorithm}[h]
\caption{\Ours}
\label{alg:main}
\begin{algorithmic}[1]
\Inputs{Training samples $(x_1, y_1), \ldots, (x_n, y_n)$, total epochs $T$, initial DNN $f_0$, $k$, $\eta > 0$}
\Outputs{$f_{T}$: trained DNN}
\Initialize{Set $\bd_{1}$ as an $n$-dimensional $k$-hot vector}
\For {epochs $t=1, \ldots, T$}
 \State Obtain $f_t$ by training $f_{t-1}$ with the $k$-set, $\bd_{t}$.
  \State Receive the noisiness feedback of each sample:
  $\theta_{1,t}, \ldots, \theta_{n,t}$.
  %\begin{align}
  %    \theta_{i,t} = \frac{1- %\mathrm{is}(f_t(x_i)= %y_i)p(f_t(x_i))}{2}
  %\end{align}
  \State Sample the perturbation ${r}_{i} \sim \mathcal{N}(0,1)$ for all $i$.
  \State Select the next $k$-set of samples: \begin{align}\label{align:FPLupdate}
  \bd_{t+1}=\argmin_{\bd \in\mathcal{D}} \left(\sum^{t}_{\tau=1} \bd \cdot \btheta_\tau + \eta \bd \cdot \boldsymbol{r}  \right)
  \end{align}
\EndFor
\end{algorithmic}
\end{algorithm}
%\subsection{Whole procedure of \Ours-based training algorithm}
%As can be seen from Algorithm~\ref{alg:main},
%the proposed method can be easily implemented
%because it is completely isolated from
%the DNN architecture. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% old version of the section of Adaptive k-set selection
\subsection{Adaptive $k$-set selection}
\label{subsec:kset}
The proposed method utilizes the idea of {\em adaptive $k$-set selection}~\cite{warmuth2008randomized}, which is a task of predicting some good $k$ elements from $n$ elements {\em repeatedly}. More specifically, its standard procedure can be formalized as follows: At each round $t$,
\begin{enumerate}
\item Select (promising) $k$ elements from $n$ elements by a selection algorithm. 
\item Receive the feedback $\theta_{1,t},\ldots,\theta_{n,t}$, as the evaluation of the selection, where $\theta_{i,t}\in [0,1]$ for all $i$.
\end{enumerate}
Formally, the selection is represented as an $n$-dimensional $k$-hot vector, $\bd_t$
and the feedback as an $n$-dimensional vector $\btheta_t$. 
The selection algorithm utilizes the previous feedback $\btheta_{t-1}$ to find the promising elements. After $T$ rounds, the selection performance is evaluated by the
{\em total selection risk} $\sum_{t=1}^T \bd_t \cdot \btheta_t$.
\par
%
The above repetitive $k$-set selection procedure assumes a dynamic process where the feedback for the selection changes along with $t$. In fact, our DNN training task is a very good example of the dynamic process because the evaluation (i.e., feedback) for each sample will change epoch-by-epoch, although the adaptive $k$-set selection has never been applied to the task.
\par
%
The theoretical highlight of adaptive $k$-set selection
is that its \emph{regret} $R_T$ can be upper bounded:
\begin{align}
R_T = \sum_{t=1}^T \bd_t \cdot \btheta_t
- \min_{\bd \in \mathcal{D}} \sum_{t=1}^T
\bd \cdot \btheta_t,
\end{align}
where $\mathcal{D}$ is the set of all possible $n$-dimensional
$k$-hot vectors (i.e., $\mathcal{D} = \{\bd \in \{0,1\}^n | \sum_{i=1}^n d_i = k\}$). %The first term $\sum_{t=1}^T \bd_t \cdot \bell_t$ is the total loss incurred by our actual selections $\bd_1,\ldots,\bd_T$. 
The first term is the total selection risk of the selection algorithm.
The second term is the total selection risk when we use {\em the best selection} at all $T$ rounds. Therefore, the regret is interpreted as the extent to which our selections are worse than the best selection. \par

The following three points should be emphasized regarding the above regret upper bound. First, $R_T$ can be bounded theoretically even though the best selection is only known after the end of the $T$ rounds and thus unknown when we decide $\bd_t$ at each $t<T$. Second, $R_T$ is still bounded even though the feedback $\theta_{i,t}$ is not predictable at all\footnote{For example, $\theta_{i,t}$ can be very large even if $\theta_{i,t-1}$ is very small. It might happen in the DNN training where just one epoch training makes a big change in the evaluation of the $i$th sample.}. Third, the upper bound of $R_T$ depends on the choice of the selection algorithm. 
For example, the {\em Follow-the-Perturbed-Leader} (FPL) algorithm achieves a good regret bound~\cite{warmuth2008randomized,koolen2010hedging,suehiro2012online,cohen2015following}, as detailed later.
\par
Despite the above interesting properties, the adaptive $k$-set selection is mainly focused on in theoretical research, and its applicability to real-world tasks has not demonstrated.
In fact, it was originally proposed for theoretical research for the online PCA task~\cite{warmuth2008randomized}. Then, many extended research studies have been proposed~\cite{koolen2010hedging,suehiro2012online,cohen2015following}, and it is still the subject of theoretical research. Therefore, this paper is the first attempt at using adaptive $k$-set selection for noisy-labeled data.\par
